Rank-DistiLLM: Closing the Effectiveness Gap Between Cross-Encoders and LLMs for Passage Re-Ranking

Cross-encoders distilled from large language models (LLMs) are often more effective re-rankers than cross-encoders fine-tuned on manually labeled data. However, distilled models do not match the effectiveness of their teacher LLMs. We hypothesize that this effectiveness gap is due to the fact that previous work has not applied the best-suited methods for fine-tuning cross-encoders on manually labeled data (e.g., hard-negative sampling, deep sampling, and listwise loss functions). To close this gap, we create a new dataset, Rank-DistiLLM. Cross-encoders trained on Rank-DistiLLM achieve the effectiveness of LLMs while being up to 173 times faster and 24 times more memory efficient. Our code and data is available at https://github.com/webis-de/ECIR-25.

==> table-dataset-characteristics.tex <==
\begin{table*}
  \centering
  \small
  % \renewcommand{\arraystretch}{0.8}%
  \setlength{\tabcolsep}{1.6pt}%
  \caption{Overview of the corpora and tasks used for evaluation. For each corpus, we report the mean document length (of the top 100 retrieved by BM25), the number of queries, and the average judgments per query.}
  % \vspace{-2ex}
  \begin{tabular}{@{}llrrrr@{}}
    \toprule
    \bfseries Corpus & \multicolumn{2}{c}{\bfseries Tasks}                                                                        & \multicolumn{2}{c}{\bfseries Queries} & \bfseries Documents                \\
    \cmidrule(r@{-0.5em}@{\tabcolsep}){2-3}  \cmidrule(l@{\tabcolsep}r@{\tabcolsep}){4-5} \cmidrule(l@{\tabcolsep}){6-6}
                     & Details                                                                                                    & \#                                    & Judg.               & \#  & Length \\
    \midrule
    Antique          & QA Benchmark~\footnotesize{~\cite{hashemi:2020}}                                                           & 1                                     & 32.9                & 200 & 49.9   \\
    Args.me          & Touch{\'e}~\footnotesize{~\cite{bondarenko:2021,bondarenko:2022}}                                          & 2                                     & 60.7                & 99  & 435.5  \\
    ClueWeb09        & Web Tracks~\footnotesize{~\cite{clarke:2009,clarke:2010,clarke:2011,clarke:2012}}                          & 4                                     & 421.8               & 200 & 1132.6 \\
    ClueWeb12        & Web Tracks, Touch{\'e}~\footnotesize{~\cite{thompson:2013,thompson:2014, bondarenko:2021,bondarenko:2022}} & 4                                     & 163.8               & 200 & 5641.7 \\
    CORD-19          & TREC-COVID~\footnotesize{~\cite{voorhees:2020,wang:2020}}                                                  & 1                                     & 1386.4              & 50  & 3647.7 \\
    Cranfield        & Fully Judged Corpus~\footnotesize{~\cite{cleverdon:1991}}                                                  & 1                                     & 8.2                 & 225 & 234.8  \\
    Disks4+5         & TREC-7/8, Robust04~\footnotesize{~\cite{voorhees:1998,voorhees:1999, voorhees:1996,voorhees:2004}}         & 3                                     & 1367.4              & 350 & 749.3  \\
    GOV              & TREC Web Tracks~\footnotesize{~\cite{craswell:2002,craswell:2003,craswell:2004}}                           & 3                                     & 603.9               & 325 & 2700.5 \\
    GOV2             & TREC TB~\footnotesize{~\cite{clarke:2004,clarke:2005,buttcher:2006}}                                       & 3                                     & 902.3               & 150 & 2410.3 \\
    MEDLINE          & Genom., PM~\footnotesize{~\cite{hersh:2004,hersh:2005,roberts:2017,roberts:2018}}                          & 4                                     & 518.3               & 180 & 309.1  \\
    MS~MARCO         & TREC DL~\footnotesize{~\cite{craswell:2019,craswell:2020}}                                                 & 2                                     & 212.8               & 97  & 77.1   \\
    NFCorpus         & Medical LTR Benchmark~\footnotesize{~\cite{boteva:2016}}                                                   & 1                                     & 48.7                & 325 & 364.6  \\
    Vaswani          & Scientific Abstracts                                                                                       & 1                                     & 22.4                & 93  & 51.3   \\
    WaPo             & Core '18                                                                                                   & 1                                     & 524.7               & 50  & 713.0  \\
    \bottomrule
  \end{tabular}
  \label{tbl-dataset-characteristics}
\end{table*}

